Mammo-CLIP: A Vision Language Foundation Model to Enhance Data Efficiency and Robustness in Mammography

The lack of large and diverse training data on Computer-Aided Diagnosis (CAD) in breast cancer detection has been one of the concerns that impedes the adoption of the system. Recently, pre-training with large-scale image text datasets via Vision-Language models (VLM) (\eg CLIP) partially addresses the issue of robustness and data efficiency in computer vision (CV). This paper proposes Mammo-CLIP, the first VLM pre-trained on a substantial amount of screening mammogram-report pairs, addressing the challenges of dataset diversity and size. Our experiments on two public datasets demonstrate strong performance in classifying and localizing various mammographic attributes crucial for breast cancer detection, showcasing data efficiency and robustness similar to CLIP in CV. We also propose Mammo-FActOR, a novel feature attribution method, to provide spatial interpretation of representation with sentence-level granularity within mammography reports. Code is available publicly: \url{https://github.com/batmanlab/Mammo-CLIP}.

==> sections/abstract_v1.tex <==
Breast cancer is a major health challenge, responsible for 670,000 deaths globally in 2022. To combat this, we introduce Mammo-CLIP, a pioneering vision-language model (VLM) pre-trained on mammogram report pairs, aimed at enhancing the computer-aided diagnosis (CAD) of breast cancer. Traditional CAD systems struggle with limited training data diversity and size. Mammo-CLIP overcomes these obstacles by leveraging dual data augmentation and multi-view supervision to enrich data diversity and volume, enhancing model generalizability. Additionally, our novel feature attribution method, CLIP-FActOR, improves interpretability by linking image features with textual findings. This approach addresses the crucial needs in radiology for generalizability, interpretability, data efficiency, and weak supervision, setting new standards in the application of AI in breast cancer diagnosis. Code is available publicly: \url{https://github.com/annonymous-vision/miccai}

==> sections/abstract_v2.tex <==
Breast cancer is the leading cancer type, characterized by high mortality rates.
Significant challenges attributed to the diversity, size, and robustness of the training datasets impede the use of Computer-Aided Diagnosis (CAD) systems in this field.
Vision-Language Models (VLMs), pre-trained on extensive collections of image-text pairs, have taken significant strides in addressing the issues of robustness and generalizability. The paper introduces Mammo-CLIP, the first VLM for mammographic analysis. Mammo-CLIP uses both mammogram-report and mammogram-finding attribute datasets to learn rich representations from limited dataset sizes. Also, we propose Mammo-FActOR, a novel feature attribution method, improving interpretability by mapping visual representations with textual findings. Through extensive experiments across 2 publicly available datasets on a range of classification and localization tasks, our method exhibits data efficiency and robustness. Code is available publicly\footnote{We will release the model checkpoints upon decision}: \url{https://github.com/annonymous-vision/miccai}

==> sections/introduction_v1.tex <==
% 1page
Vision-language models (VLMs) have catalyzed a transformative leap in bridging the realms of computer vision and natural language processing, setting new benchmarks for understanding and interaction across diverse modalities. 
VLMs harness large image-text pair datasets, leveraging captions to identify key image representations. Applications of VLMs include superior zero-shot and label-efficient classification~\cite{radford2021learning, li2022supervision, jia2021scaling, wang2021efficientclip}, constructing label free interpretable models~\cite{oikarinen2023label, yang2023language}, discovering error slices of classifiers~\cite{zhang2023diagnosing, eyuboglu2022domino, slyman2023vlslice}. In medicine, the availability of extensive CXR-report pairs like MIMIC-CXR~\cite{johnson2019mimic} primarily leads the development of VLMs in the chest X-ray (CXR) domain~\cite{zhang2022convirt, huang2021gloria, wu2023medklip, wang2022medclip, you2023cxr}. Other domains mostly rely on VLMs created using image text captions from PubMed or public forms~\cite{kim2023fostering, lin2023pmc, huang2023visual}. This paper introduces Mammo-CLIP, a novel VLM trained with breast mammogram-report and mammogram-findings pairs. Also, we propose CLIP-Factor -- CLIP for \underline{\textbf{F}}eature \underline{\textbf{A}}ttribution \underline{\textbf{C}}onnecting \underline{\textbf{O}}bservations and \underline{\textbf{R}}eports, a novel feature attribution method aligning the image representation with textual findings.


VLM has good representation across many tasks \cite{radford2021learning}.
Downstream zs, LP, and FT. Chest/Generic image-caption PMC. clip Applications, bias detection domino kind


2nd para: Why do we need VLM for med img? text is weak sup, text can be grounding. robustness

3rd Gap:
expensive data collection
Creating VLMs for mammograms encounters unique challenges, such as the scarcity and cost of accurate annotations by medical professionals due to privacy and legal concerns, the smaller scale of datasets in comparison to typical image-text pairs in computer vision, and the lack of efficient methods for associating visual features with textual attributes in reports. 

one way use clip reduce dimension, create clip by finetuing, create organ specific clip
low image breast. GAP create clip by finetuing, utility of MVS: low image-text

Why MVS:
% excerpt from Declip
% We argue that these prior arts only use the single image-text contrastive supervision while overlooking the
% widespread supervision within the pairs, thus is inefficient.
% Firstly, there underlies rich structural information within each modality itself (LeCun & Misra,
% 2021). We can tweak some words/pixels in a sentence/image while retaining a similar semantic
% meaning. This sort of self-supervision can be exploited to learn a more common-sense representation for each modality (Devlin et al., 2018; He et al., 2020; Chen et al., 2020a). Moreover, inspired
% by contrasting multi-crops in an image (Caron et al., 2020), we further extend the multi-view 1
% supervision into our multi-modality setting. Specifically, each image is paired with multiple textual
% descriptions obtained via stochastic augmentations, vice versa. The benefit is intuitive: this auxiliary
% multi-view supervision brings more invariant and robust information.
lit - review

Gap: 

Full form of (MVS and SS, CXR, VLM)

Prev work on VILLA and R-clip

No Breast clip. 

The image-text dataset is small, we can augment it with the help of image-label dataset. 

No feature attribution method based on the text on the report. Where does the image look at for mass based on text?

Contribution:
Inhouse dataset image-text.Augment datasets synthesize reports, handling large image size
1. Propose Breast-CLIP - 1st ever image text

2. Tackled the problem of less image-text data by augmenting the dataset with image labels datasets

3. Comprehensive evaluation on classification of mass, calc, density and cancer across two public dataset, object detection

4. Present a novel feature attribution method based on text from report. CLIP for \underline{F}eature \underline{A}ttribution \underline{C}onnecting \underline{O}bservations and \underline{R}eports (CLIP-Factor)


% Our methodology integrates three key components designed to enhance the analysis of mammogram-report pairs, specifically tailored for working with constrained dataset sizes common in medical imaging studies. The components are as follows:

% Dual Data Augmentation Strategy: Initially, we expand each study's mammogram-report pair to capture a wider array of imaging and textual semantics. This is achieved by applying a two-fold augmentation process: first, directly augmenting the existing mammogram-report pairs, and subsequently, enriching the dataset by integrating mammogram-attribute data. This dual approach allows us to significantly increase the diversity and volume of our training data, addressing the common issue of dataset scarcity in medical imaging fields.

% Pre-training with MVS Loss Function: To effectively leverage the augmented dataset, we employ a Multi-View Supervision (MVS) loss function during the pre-training phase. This strategy is designed to extract superior representations from the augmented, yet relatively small, dataset. By utilizing MVS, we ensure that the model learns to generalize across a variety of imaging and textual contexts, thereby enhancing its performance and reliability.

% Novel Feature Attribution Method: The final component of our approach focuses on interpretability, a critical aspect of medical imaging AI applications. We introduce a novel feature attribution method that systematically maps textual attributes to visual features extracted by the image encoder. This mapping not only aids in understanding the model's decision-making process but also provides valuable insights into the correlation between textual findings and their corresponding imaging features, enhancing the model's utility for medical professionals.

==> sections/introduction_v2.tex <==
% 1page
Vision-language models (VLMs) have catalyzed a transformative leap in bridging the realms of computer vision and natural language processing, setting new benchmarks for understanding and interaction across diverse modalities. 
VLMs harness large image-text pair datasets, leveraging captions to identify key image representations. Applications of VLMs include superior zero-shot and label-efficient classification~\cite{radford2021learning, li2022supervision, jia2021scaling, wang2021efficientclip}, constructing label free interpretable models~\cite{oikarinen2023label, yang2023language}, discovering error slices of classifiers~\cite{zhang2023diagnosing, eyuboglu2022domino, slyman2023vlslice}. In medicine, the availability of extensive CXR-report pairs like MIMIC-CXR~\cite{johnson2019mimic} primarily leads the development of VLMs in the chest X-ray (CXR) domain~\cite{zhang2022convirt, huang2021gloria, wu2023medklip, wang2022medclip, you2023cxr}. Other domains mostly rely on VLMs created using image text captions from PubMed or public forms~\cite{kim2023fostering, lin2023pmc, huang2023visual}. This paper introduces Mammo-CLIP, a novel VLM trained with breast mammogram-report and mammogram-findings pairs. Also, we propose CLIP-Factor -- CLIP for \underline{\textbf{F}}eature \underline{\textbf{A}}ttribution \underline{\textbf{C}}onnecting \underline{\textbf{O}}bservations and \underline{\textbf{R}}eports, a novel feature attribution method aligning the image representation with textual findings. Our method is the first to develop and interpret a VLM in breast imaging domain.

\noindent In medicine, texts can be deemed as weak labels for disease localization~\cite{yu2022anatomy}, interpretability~\cite{ghosh2023dividing, ghosh2023distilling}, grounding~\cite{chen2023medical} and robustness~\cite{eslami2021does, liu2023clip}. However, the scarcity and cost of annotations by medical professionals due to privacy and legal concerns often impede the development of VLMs for mammograms. A naive strategy for developing Mammo-CLIP involves adapting the CLIP model through fine-tuning. This process requires lowering the image resolution to match CLIP's input specifications. Yet, such transformations lose the crucial semantic details embedded in high-resolution mammograms essential for accurate interpretation and diagnosis. Moreover, the dataset comprising mammogram-report pairs is considerably smaller than the one utilized to train CLIP. Also, we lack a method to capture the representations for a given finding via textual description.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{plots/main/Schematic.pdf}
\caption{Schematic view of our method. (to be updated)}
\label{fig:schematic}
\end{center}
\end{figure*}

\noindent\textbf{Contribution.} Our contributions are summarized as follows:
\ding{182} We present Mammo-CLIP to enhance the analysis of mammogram-report pairs, specifically tailored for working with constrained dataset sizes common in medical imaging studies. \underline{We utilize
dual data augmentation strategy.} Initially, we expand each study's mammogram-report pair to capture a wider array of imaging and textual semantics. This is achieved by applying a two-fold augmentation process: first, directly augmenting the existing mammogram-report pairs and, subsequently, enriching the dataset by integrating mammogram-attribute data. This dual approach allows us to significantly increase the diversity and volume of our training data, addressing dataset scarcity in medical imaging fields.
\underline{We pre-train Mammo-CLIP with
multi-view supervision (MVS)}. To leverage the augmented dataset effectively, we employ a MVS loss function during the pre-training phase. This strategy is designed to extract superior representations from the relatively small, augmented dataset. By utilizing MVS, we ensure the model learns to generalize across various imaging and textual contexts, enhancing its performance and reliability.
\ding{183} We present CLIP-Factor. The final component of our approach focuses on interpretability, a critical aspect of medical imaging AI applications. We introduce a novel feature attribution method that systematically maps textual attributes to visual features extracted by the image encoder. This mapping not only aids in understanding the model's decision-making process but also provides valuable insights into the correlation between textual findings and their corresponding imaging features, enhancing the model's utility for medical professionals.

==> sections/introduction_v3.tex <==
% 1page
Vision-language models (VLMs) initiate a transformative leap in bridging the realms of computer vision and natural language processing, setting new benchmarks for understanding and interaction across diverse modalities. Applications of VLMs include superior zero-shot and label-efficient classification~\cite{radford2021learning, li2022supervision, jia2021scaling, wang2021efficientclip}, constructing label free interpretable models~\cite{oikarinen2023label, yang2023language}, discovering error slices of classifiers~\cite{zhang2023diagnosing, eyuboglu2022domino, slyman2023vlslice}. In medicine, the availability of extensive CXR-report pairs like MIMIC-CXR~\cite{johnson2019mimic} leads the development of VLMs in the chest X-ray (CXR) domain~\cite{zhang2022convirt, huang2021gloria, wu2023medklip, wang2022medclip, you2023cxr}. Other domains mostly rely on VLMs created using images and captions from PubMed or public forums~\cite{kim2023fostering, lin2023pmc, huang2023visual}. This paper introduces Mammo-CLIP, the first VLM trained with breast mammogram-report and mammogram-findings pairs of patients. Also, we propose CLIP-Factor -- CLIP for \underline{\textbf{F}}eature \underline{\textbf{A}}ttribution \underline{\textbf{C}}onnecting \underline{\textbf{O}}bservations and \underline{\textbf{R}}eports, a novel feature attribution method aligning the image representation with textual findings. 
% Our method is the first to develop and interpret a VLM in breast imaging domain.

 In medicine, texts can be deemed as weak labels for disease localization~\cite{yu2022anatomy}, interpretability~\cite{ghosh2023dividing, ghosh2023distilling}, grounding~\cite{chen2023medical} and robustness~\cite{eslami2021does, liu2023clip}. However, the scarcity and cost of annotations by medical professionals due to privacy and legal concerns often impede the development of VLMs for mammograms. A naive strategy for developing Mammo-CLIP involves adapting the CLIP model through fine-tuning. This process requires lowering the image resolution to match CLIP's input specifications. Yet, such transformations lose the crucial semantic details embedded in high-resolution mammograms essential for accurate interpretation and diagnosis. Moreover, the dataset comprising mammogram-report pairs is considerably smaller than the one utilized to train CLIP. Also, we lack a method to capture the representations for a given finding via textual description.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{plots/main/Schematic.pdf}
\caption{Schematic view of our method. (to be updated)}
\label{fig:schematic}
\end{center}
\end{figure*}

\noindent\textbf{Contribution.} Our contributions are summarized as follows:
\ding{182} We present Mammo-CLIP to enhance the analysis of mammogram-report pairs, specifically tailored for working with constrained dataset sizes common in medical imaging studies. \underline{We utilize
dual data augmentation strategy.} Initially, we expand each study's mammogram-report pair to capture a wider array of imaging and textual semantics. This is achieved by applying a two-fold augmentation process: first, directly augmenting the existing mammogram-report pairs and, subsequently, enriching the dataset by integrating mammogram-attribute data. This dual approach allows us to significantly increase the diversity and volume of our training data, addressing dataset scarcity in medical imaging fields.
\underline{We pre-train Mammo-CLIP with
multi-view supervision (MVS)}. To leverage the augmented dataset effectively, we employ a MVS loss function during the pre-training phase. This strategy is designed to extract superior representations from the relatively small, augmented dataset. By utilizing MVS, we ensure the model learns to generalize across various imaging and textual contexts, enhancing its performance and reliability.
\ding{183} We present CLIP-Factor. The final component of our approach focuses on interpretability, a critical aspect of medical imaging AI applications. We introduce a novel feature attribution method that systematically maps textual attributes to visual features extracted by the image encoder. This mapping not only aids in understanding the model's decision-making process but also provides valuable insights into the correlation between textual findings and their corresponding imaging features, enhancing the model's utility for medical professionals.

==> sections/introduction_v4.tex <==
% 1page
Breast cancer remains a leading cause of mortality among women, with a global death toll of 670,000 in 2022. Creating AI tools to identify cancer in mammograms has been a central focus for computer-aided diagnosis (CAD)~\cite{alberdi2005use, srivastava2013design, srivastava2014quantitative}. Implementing CAD for breast cancer is clinically challenging due to the training data's robustness, diversity, and size~\cite{chan2019cad}. Vision-language models (VLM) \eg CLIP~\cite{radford2021learning}, pre-trained on large image-text pairs, partially tackle robustness and generalizability issues in computer vision (CV). The lack of image-text datasets due to annotation cost impedes the development of such models in mammography. This paper introduces Mammo-CLIP, the first VLM trained with breast mammogram-report and mammogram-findings pairs of patients. Also, Additionally, we propose CLIP-FActOR -- CLIP for \underline{\textbf{F}}eature \underline{\textbf{A}}ttribution \underline{\textbf{C}}onnec\underline{\textbf{T}}ing \underline{\textbf{O}}bservations and \underline{\textbf{R}}eports, novel feature attribution technique, enhancing interpretability by aligning image representations with textual findings.


VLMs align image-text representations in joint embedding space, providing significant advantages. Pretraining on extensive datasets enhances generalizability~\cite{eslami2021does, liu2023clip}. The language encoder reduces reliance on costly attribute annotations for developing interpretable models~\cite{yang2023language, oikarinen2023label}. Also, it demonstrates data-efficiency~\cite{radford2021learning, li2022supervision, jia2021scaling}. In medical imaging, texts from radiology reports serve as a source of weak labels, aiding disease localization~\cite{yu2022anatomy, han2022radiomics, muller2023anatomy}. These characteristics --generalizability, interpretability, data efficiency, and weak supervision -- are crucial for medical imaging applications, improving diagnostic precision and insightful analysis.


In medical imaging, the availability of extensive chest X-ray-report pairs like MIMIC-CXR~\cite{johnson2019mimic} fuels the construction of VLMs~\cite{zhang2022convirt, huang2021gloria, wu2023medklip, wang2022medclip, you2023cxr}. Other domains mostly rely on VLMs created using images and captions from PubMed or public forums~\cite{kim2023fostering, lin2023pmc, huang2023visual}. Thus, a naive strategy for developing Mammo-CLIP involves fine-tuning the CLIP model. This process lowers the image resolution to match CLIP's input dimensions. Such transformations lose the semantic visual cues embedded in high-resolution mammograms essential for accurate interpretation and diagnosis. Also, we lack a method to capture the representations for a given finding \eg \textit{mass}, \textit{calcification} \etc~via textual description.


% Moreover, the dataset comprising mammogram-report pairs is considerably smaller than the one utilized to train CLIP. 

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{plots/main/Schematic.pdf}
\caption{Schematic view of our method. (to be updated)}
\label{fig:schematic}
\end{center}
\end{figure*}

\noindent\textbf{Contribution.} Our contributions are summarized as follows:
(1) We present Mammo-CLIP, the first VLM pre-trained using mammogram-report pairs specifically suited for limited dataset sizes common in medical imaging studies. (2) We introduce CLIP-FActOR.
Mammo-CLIP utilizes
dual data augmentation strategy and multi-view supervision (MVS)~\cite{li2022supervision}. The dual augmentation technique diversifies each mammogram-report pair, enhancing the range of captured imaging and textual semantics.  This dual approach allows us to significantly increase the diversity and volume of our training data, addressing dataset scarcity in mammography.
Next, the pre-training phase employs an MVS loss function. This strategy extracts superior representations from the relatively small, augmented dataset. 
% MVS ensures the model to generalize across various imaging and textual contexts, enhancing its performance and reliability.
The final contribution, CLIP-FActOR, focuses on interpretability. This novel feature attribution method systematically maps textual attributes to image-encoder-extracted visual representations. This mapping aids medical practitioners in understanding the model's decision-making process and discovering valuable insights.

First, we utilize the learned representations of
Mammo-CLIP in image classification tasks across two publicly available datasets

==> sections/method_v1.tex <==
% one line present notation, augmentation, MVS and SS loss. and feature - clip method. For brevity we denote $A$ for augmentation function for both image and text.

% 2 page

% $N$ study-report pair

% $\boldsymbol{x^I}$ and $\boldsymbol{x^T}$

% $\boldsymbol{f^I}$ and $\boldsymbol{f^T}$

% $\boldsymbol{z^I}$ and $\boldsymbol{z^T}$
\textbf{Notation.}
Assume \{($\boldsymbol{x^I_i}, \boldsymbol{x^T_i}$)\} is an image-text pair of the $i^{th}$ study. Fig. illustrates our approach. In following section, we present the augmentation strategy for MVS, the loss function to conduct the pre-training and the feature attribution method to discover the correspondence between imaging features and textual findings. 

\subsection{Dataset augmentation}
\label{sec:dataset_aug}
\noindent\textbf{Augmenting image-text pairs with image-label pairs.} 
 High-quality annotations from medical specialists are expensive to obtain due to privacy and legal concerns. As a result
paired mammography image-text datasets are significantly smaller than general paired image-text datasets in vision. Inspired by previous works on the CXR domain~\cite{huang2021gloria, you2023cxr}, we augment the image-text dataset with the existing image-label datasets. For an arbitrary image $\boldsymbol{x^I} \in \mathcal{X}$, the image-label dataset includes multi-hot finding attributes $y \in \mathcal{Y}$, \eg \textit{mass, calcification,} \etc instead of $\boldsymbol{x^T}$. We synthesize the report for $\boldsymbol{x^I}$ as $\boldsymbol{x^T} = \text{Concat}({p \sim P(y)}_{y \in \mathcal{Y}})$, where $p, P(y)$ and $Concat(.)$ denotes a sampled prompt sentence, a set of prompts corresponding to attributes, and the concatenation of texts respectively. A board-certified radiologist develops a set of prompts for different attributes and their values (positive, negative, etc.). Our prompts are available in the Appendix.

\noindent\textbf{Augmenting for MVS.}
Despite synthesizing reports, the dataset size remains significantly smaller than CLIP's. We tackle this by utilizing the MVS strategy. MVS employs self-supervision across four pairs: ($\boldsymbol{x^I}, \boldsymbol{x^T}$), ($\boldsymbol{x^I}, A(\boldsymbol{x^T})$), ($A(\boldsymbol{x^I}), \boldsymbol{x^T}$), and ($A(\boldsymbol{x^I}), A(\boldsymbol{x^T})$). For brevity, we denote $A$ for image and text augmentation. We capture different imaging semantics of a study by utilizing CC and MLO views of breast mammography for $\boldsymbol{x^I}$ and $A(\boldsymbol{x^I})$, respectively. Similarly, we employ the impression and findings sections of the mammography report as $\boldsymbol{x^T}$ and $A(\boldsymbol{x^T})$, respectively, to harness various textual semantics. If a study lacks either both views or both sections of the report, we apply similar image and text augmentations as done in previous works~\cite{you2023cxr, li2022supervision}.


\subsection{Loss function}

\noindent\textbf{InfoNCE loss.} CLIP~\cite{radford2021learning} aligns the representations of images and texts in a shared high-dimensional space by pulling the paired image and text embeddings closer and pushing the unpaired image and text embeddings further.  
Let $\boldsymbol{z^I} \in \boldsymbol{Z^I}$ and $\boldsymbol{z^T} \in \boldsymbol{Z^T}$ are the normalized image and text embeddings, obtained from $f^I(.)$ and $f^T(.)$ -- the image and text encoders respectively. We denote the $i^{th}$ paired image-text representation as $\{\boldsymbol{z^I_i, z^T_i}\}$.
For a batch size of $|B|$, CLIP utilizes the following InfoNCE loss to update the image encoder,

\begin{equation}
\label{equ: INFO_NCE}
L^{I->T}_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T}) = -\frac{1}{N}\big( 
    \sum_{i=1}^{|B|} \log \frac{\text{exp}(<\boldsymbol{z_i^I}, \boldsymbol{z_i^T}>/\tau)}{\sum_{j=1}^N \text{exp}(<\boldsymbol{z_i^I}, \boldsymbol{z_j^T}>/\tau)}  
\big) ,
\end{equation}

where $<.,.>$ denotes the similarity function and $\tau$ is a learnable temperature to scale the logits. CLIP has a bidirectional symmetrical loss to update the image and text encoders with the overall loss function as,

\begin{equation}
\label{equ: INFO_NCE}
L_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T}) = \frac{L^{I->T}_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T}) + L^{T->I}_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T})}{2}
\end{equation}


\noindent\textbf{MVS loss.}
To mitigate the issue of dataset size in mammograms, MVS utilizes cross-modal self-supervision of every pair of original and augmented image-text pairs. We denote  $\boldsymbol{\Tilde{z}^I} \in \Tilde{\boldsymbol{Z}}^I$ and $\boldsymbol{\Tilde{z}^T} \in \Tilde{\boldsymbol{Z}}^T$, as the normalized image and text embeddings of augmented image and text respectively. Thus, the MVS loss is,

\begin{equation}
L_{MVS} = \frac{1}{4}(
    L_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T})+
    L_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{\Tilde{Z}^T})+
    L_{CLIP}(\boldsymbol{\Tilde{Z}^I}, \boldsymbol{Z^T})+
    L_{CLIP}(\boldsymbol{\Tilde{Z}^I}, \boldsymbol{\Tilde{Z}^T})
)
\end{equation}

\noindent\textbf{SS loss}
MVS aligns representations across modalities. To align representations within modalities, we utilize SS loss~\cite{you2023cxr, boecking2022making}. Specifically, we construct the SS loss as $L_{ISS} = L_{CLIP}(\boldsymbol{Z}^I, \boldsymbol{\Tilde{Z}^I})$ and $L_{TSS} = L_{CLIP}(\boldsymbol{Z}^T, \boldsymbol{\Tilde{Z}^T})$ to align image and text representations respectively. $L_{ISS}$ pulls the image embeddings from the same study and pushes the same for different studies. $L_{TSS}$ performs the same for text embeddings. \textbf{Overall loss.} Thus we optimize the total pre-training objective as: $L = L_{MVS} + \lambda_IL_{ISS} + \lambda_TL_{TSS}$


\subsection{Discovering correspondence between imaging features and textual finding}
% Grounding, Weak Sup, 
VLM encourages grounding of the image representations to the textual embeddings. In other words, these textual embeddings can be deemed as weak labels of the finding labels, \eg \textit{mass, calcification} \etc       We argue that the image representations, obtained from VLM has a many-to-many correspondence to the finding attributes via textual descriptions from the report. In a image-label dataset $\{\boldsymbol{x}_i, \boldsymbol{y}_i\}_{i=1}^N$, assume $\boldsymbol{x}_i$ and $\boldsymbol{y}_i$ denote the image and $K$-hot vector indicating values of $K$ finding attributes respectively for the $i^{th}$ sample.
Also, $\sigma(f^I(\boldsymbol{x_i})) \in \mathbb{R}^{c \times hw}$ is the image representation, where $\sigma$ resizes the representations from $\mathbb{R}^{c \times h \times w}$ to $\mathbb{R}^{c \times hw}$. We denote the mapping function, $\pi^k: \mathbb{R}^{c \times hw} \rightarrow \mathbb{R}^{c \times d}$, signifying the correspondence between a finding attribute $k \in \boldsymbol{y}$ attribute and image representations. Here $d$ denotes the output embedding dimensions. For an arbitrary sample, we generate the embeddings of the textual findings of $k^{th}$ attribute, denoted as $\boldsymbol{t^k_i} \in \mathbb{R}^{d}$, from $f^T(.)$ using the positively mentioned prompts, described in Sec. \ref{sec:dataset_aug}. 
\textbf{Training.} Given the frozen image and text encoders $\{f^I(.)$, $f^T(.)\}$ and $\{\pi^k, \boldsymbol{t^k}\}^K_{k=1}$, we train all the $\pi^k$s using the following contrastive loss,

\begin{equation}
L_(\boldsymbol{x_i, y_i}) = -\sum_{k \in \boldsymbol{y_i}}\log
\frac{
    \phi(\pi^k(\sigma(f^I(\boldsymbol{x_i}))), \boldsymbol{t_i}^k)
}
{
    \phi(\pi^k(\sigma(f^I(\boldsymbol{x_i}))), \boldsymbol{t_i}^k) +
    \sum^{|B|}_{j=1; k\notin \boldsymbol{y_j}}\phi(\pi^k(\sigma(f^I(\boldsymbol{x_j}))), \boldsymbol{t_i}^k)
},
\end{equation}

where $\phi = \exp(\max(<a,b>)/\tau)$. For a image $(\boldsymbol{x_i}, \boldsymbol{y_i})$ and a finding attribute $k\in\boldsymbol{y}_i$, this loss encourages  the maximum pairwise similarity between
the embedding of image representation $\pi^k(\sigma(f^I(\boldsymbol{x_i})))$ and the attribute embedding $t^k_i$ to be high, since at least one feature in $f^I(\boldsymbol{x}_i)$ depicts attribute
$k$. 
Simultaneously, for an image $\boldsymbol{x_j}$ where $k \notin \boldsymbol{y}_j$ , the maximum pairwise similarity between the 
$\pi^k(\sigma(f^I(\boldsymbol{x_j})))$ and the attribute embedding $t^k_i$
is encouraged to be
low, since no features in $f^I(\boldsymbol{x}_j)$ depict attribute $k$.

==> sections/method_v2.tex <==
 This section describes 1) our augmentation strategy for MVS, 2) the loss function for the pre-training Mammo-CLIP, and 3) the novel feature attribution method to discover the correspondence between imaging features and textual findings. 
 Fig. illustrates our approach.
 
\subsection{Dataset augmentation}
\label{sec:dataset_aug}
\noindent\textbf{Augmenting image-text pairs with image-label pairs.} 
 High-quality annotations from medical specialists are scarce and expensive, primarily due to privacy and legal constraints.
 Consequently
paired mammogram-report datasets are notably smaller than paired image-text datasets in computer vision. Motivated from the CXR domain~\cite{you2023cxr, wang2022medclip}, we augment the image-text dataset with the existing image-label datasets. For a given image $\boldsymbol{x^I} \in \mathcal{X}$, the image-label dataset comprises a set of paired finding attributes $y \in \mathcal{Y}$, \eg \textit{mass, calcification,} \etc~instead of reports. For $\boldsymbol{x^I}$, we synthesize the report, $\boldsymbol{x^T} = \text{Concat}({p \sim P(y)}_{y \in \mathcal{Y}})$, where $p, P(y)$ and $Concat(.)$ denote a sampled prompt sentence, a set of prompts corresponding to attributes, and the concatenation of texts respectively. A board-certified radiologist develops a set of prompts for different attributes and their values (positive, negative, etc.). We include the prompts in the Appendix.

\noindent\textbf{Augmenting for MVS.}
Despite the report synthesis, the dataset remains significantly smaller than CLIP's. We tackle this with the MVS strategy. MVS employs self-supervision across four pairs: ($\boldsymbol{x^I}, \boldsymbol{x^T}$), ($\boldsymbol{x^I}, A(\boldsymbol{x^T})$), ($A(\boldsymbol{x^I}), \boldsymbol{x^T}$), and ($A(\boldsymbol{x^I}), A(\boldsymbol{x^T})$). For brevity,$A$ denotes image and text augmentation. We capture different imaging semantics of a study by utilizing CC and MLO views of breast mammography for $\boldsymbol{x^I}$ and $A(\boldsymbol{x^I})$, respectively. Similarly, we employ the impression and findings sections of the mammography report as $\boldsymbol{x^T}$ and $A(\boldsymbol{x^T})$, respectively, to harness various textual semantics. If a study lacks either both views or both sections of the report, we apply similar image and text augmentations as done in previous works~\cite{you2023cxr, li2022supervision}.


\subsection{Loss function}

\noindent\textbf{InfoNCE loss.} CLIP~\cite{radford2021learning} aligns the representations of images and texts in a shared high-dimensional space by pulling the paired image and text embeddings closer and pushing the unpaired image and text embeddings further.  
Let $\boldsymbol{z^I} \in \boldsymbol{Z^I}$ and $\boldsymbol{z^T} \in \boldsymbol{Z^T}$ are the normalized image and text embeddings, obtained from $f^I(.)$ and $f^T(.)$ -- the image and text encoders respectively. We denote the $i^{th}$ paired image-text representation as $\{\boldsymbol{z^I_i, z^T_i}\}$.
For a batch size of $|B|$, CLIP utilizes the following InfoNCE loss to update the image encoder,

\begin{equation}
\label{equ: INFO_NCE}
L^{I->T}_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T}) = -\frac{1}{N}\big( 
    \sum_{i=1}^{|B|} \log \frac{\text{exp}(<\boldsymbol{z_i^I}, \boldsymbol{z_i^T}>/\tau)}{\sum_{j=1}^N \text{exp}(<\boldsymbol{z_i^I}, \boldsymbol{z_j^T}>/\tau)}  
\big) ,
\end{equation}

where $<.,.>$ denotes the similarity function and $\tau$ is a learnable temperature to scale the logits. CLIP has a bidirectional symmetrical loss to update the image and text encoders with the overall loss function as,

\begin{equation}
\label{equ: INFO_NCE}
L_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T}) = \frac{L^{I->T}_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T}) + L^{T->I}_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T})}{2}
\end{equation}


\noindent\textbf{MVS loss.}
To alleviate the issue of dataset size in mammograms, MVS utilizes cross-modal self-supervision of every pair of original and augmented image-text pairs, learning superior representations. We denote  $\boldsymbol{\Tilde{z}^I} \in \Tilde{\boldsymbol{Z}}^I$ and $\boldsymbol{\Tilde{z}^T} \in \Tilde{\boldsymbol{Z}}^T$, as the normalized image and text embeddings of augmented image and text respectively. Thus, the MVS loss is,

\begin{equation}
L_{MVS} = \frac{1}{4}(
    L_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{Z^T})+
    L_{CLIP}(\boldsymbol{Z^I}, \boldsymbol{\Tilde{Z}^T})+
    L_{CLIP}(\boldsymbol{\Tilde{Z}^I}, \boldsymbol{Z^T})+
    L_{CLIP}(\boldsymbol{\Tilde{Z}^I}, \boldsymbol{\Tilde{Z}^T})
)
\end{equation}

\noindent\textbf{SS loss}
MVS aligns representations across modalities. To align representations within modalities, we utilize SS loss~\cite{you2023cxr, boecking2022making}. Specifically, we construct the SS loss as $L_{ISS} = L_{CLIP}(\boldsymbol{Z}^I, \boldsymbol{\Tilde{Z}^I})$ and $L_{TSS} = L_{CLIP}(\boldsymbol{Z}^T, \boldsymbol{\Tilde{Z}^T})$ to align image and text representations respectively. $L_{ISS}$ pulls the image embeddings from the same study and pushes the same for different studies. $L_{TSS}$ performs the same for text embeddings. \textbf{Overall loss.} Thus we optimize the total pre-training objective as: $L = L_{MVS} + \lambda_IL_{ISS} + \lambda_TL_{TSS}$


\subsection{Discovering correspondence between imaging features and textual finding}
% Grounding, Weak Sup, 
VLM encourages grounding of the image representations to the textual embeddings. In other words, these textual embeddings can be deemed as weak labels of the finding labels, \eg \textit{mass, calcification} \etc       We argue that the image representations, obtained from VLM has a many-to-many correspondence to the finding attributes via textual descriptions from the report. In a image-label dataset $\{\boldsymbol{x}_i, \boldsymbol{y}_i\}_{i=1}^N$, assume $\boldsymbol{x}_i$ and $\boldsymbol{y}_i$ denote the image and $K$-hot vector indicating values of $K$ finding attributes respectively for the $i^{th}$ sample.
Also, $\sigma(f^I(\boldsymbol{x_i})) \in \mathbb{R}^{c \times hw}$ is the image representation, where $\sigma$ resizes the representations from $\mathbb{R}^{c \times h \times w}$ to $\mathbb{R}^{c \times hw}$. We denote the mapping function, $\pi^k: \mathbb{R}^{c \times hw} \rightarrow \mathbb{R}^{c \times d}$, signifying the correspondence between a finding attribute $k \in \boldsymbol{y}$ attribute and image representations. Here $d$ denotes the output embedding dimensions. For an arbitrary sample, we generate the embeddings of the textual findings of $k^{th}$ attribute, denoted as $\boldsymbol{t^k_i} \in \mathbb{R}^{d}$, from $f^T(.)$ using the positively mentioned prompts, described in Sec. \ref{sec:dataset_aug}. 
\textbf{Training.} Given the frozen image and text encoders $\{f^I(.)$, $f^T(.)\}$ and $\{\pi^k, \boldsymbol{t^k}\}^K_{k=1}$, we train all the $\pi^k$s using the following contrastive loss,

\begin{equation}
L_(\boldsymbol{x_i, y_i}) = -\sum_{k \in \boldsymbol{y_i}}\log
\frac{
    \phi(\pi^k(\sigma(f^I(\boldsymbol{x_i}))), \boldsymbol{t_i}^k)
}
{
    \phi(\pi^k(\sigma(f^I(\boldsymbol{x_i}))), \boldsymbol{t_i}^k) +
    \sum^{|B|}_{j=1; k\notin \boldsymbol{y_j}}\phi(\pi^k(\sigma(f^I(\boldsymbol{x_j}))), \boldsymbol{t_i}^k)
},
\end{equation}

where $\phi = \exp(\max(<a,b>)/\tau)$. For a image $(\boldsymbol{x_i}, \boldsymbol{y_i})$ and a finding attribute $k\in\boldsymbol{y}_i$, this loss encourages  the maximum pairwise similarity between
the embedding of image representation $\pi^k(\sigma(f^I(\boldsymbol{x_i})))$ and the attribute embedding $t^k_i$ to be high, since at least one feature in $f^I(\boldsymbol{x}_i)$ depicts attribute
$k$. 
Simultaneously, for an image $\boldsymbol{x_j}$ where $k \notin \boldsymbol{y}_j$ , the maximum pairwise similarity between the 
$\pi^k(\sigma(f^I(\boldsymbol{x_j})))$ and the attribute embedding $t^k_i$
is encouraged to be
low, since no features in $f^I(\boldsymbol{x}_j)$ depict attribute $k$.

==> sections/method_v3.tex <==
% Challenges may go to the intro
Our method consists of three components: 1) a dual data augmentation strategy to augment the mammogram-report pairs of each study with different views and report-sections and subsequently, augment the dataset with mammogram-attribute dataset; 2) pre-training strategy with MVS loss to learn superior representations from a relatively smaller dataset; 3) a novel feature attribution method to map the textual attributes to the visual features of the image encoder of our Mammo-CLIP model for interpretability. We start with a image-text dataset $\{\boldsymbol{x}^I_i, \boldsymbol{x}^T_i\}_{i=1}^N$, with $N$ is the number of studies. 
Fig \ref{fig:schematic}. illustrates our approach.

\subsection{Augmentation}
\label{sec:dataset_aug}
\noindent\textbf{Image-text augmentation.}
We utilize MVS to learn from the available smaller datasets. MVS employs self-supervision across four pairs: ($\boldsymbol{x}^I, \boldsymbol{x}^T$), ($\boldsymbol{x}^I, A(\boldsymbol{x}^T)$), ($A(\boldsymbol{x}^I), \boldsymbol{x}^T$), and ($A(\boldsymbol{x}^I), A(\boldsymbol{x}^T)$). For brevity, $A$ denotes image and text augmentation. For $i^{th}$ study, $\boldsymbol{x}^I_i$ and $A(\boldsymbol{x}^I_i)$ denote the CC and MLO views respectively.  Likewise, $\boldsymbol{x}^T_i$ and $A(\boldsymbol{x}^T_i)$ denote the impression and findings sections of the report, respectively. For studies without certain views or report sections, we apply similar image and text augmentations, done in~\cite{you2023cxr, li2022supervision}.
\noindent\textbf{Dataset augmentation.} To further mitigate the challenge of the small size of mammography datasets, we synthesize reports from existing mammogram-attribute datasets. Such datasets consist of a mammogram image $\boldsymbol{x}^I$, paired with a set of finding attributes $y \in \mathcal{Y}$, \eg \textit{mass, calcification,} \etc~For $i^{th}$ sample, we synthesize the report as, $\boldsymbol{x}^T_i = \text{Concat}({p \sim P(y)}_{y \in \mathcal{Y}})$, where $p, P(y)$ and $Concat(\cdot)$ denote a sampled prompt sentence, a set of prompts corresponding to attributes, and the concatenation of texts respectively. We include the prompts, constructed by a board-certified radiologist, in the Appendix.


\subsection{Loss function}

\noindent\textbf{MVS loss for crossmodal alignment.} The MVS pre-training strategy leverages cross-modal self-supervision across both original and augmented image-text pairs, enhancing the model's ability to generalize from limited data.  
For $i^{th}$ study, $\boldsymbol{z}^I_i \in \mathcal{Z}^I$ and $\boldsymbol{z}_i^T \in \mathcal{Z}^T$ represent the normalized image and text representations, respectively for the image-text pair $(\boldsymbol{x}^I_i, \boldsymbol{x}^T_i)$.  Similarly, $\Tilde{\boldsymbol{z}}^I_i \in \Tilde{\mathcal{Z}}^I$ and $\Tilde{\boldsymbol{z}}^T_i \in \Tilde{\mathcal{Z}}^T$, denote the normalized representations of the augmented image and text, $A(\boldsymbol{x}^I_i)$ and $A(\boldsymbol{x}^T_i)$, respectively. The following optimization loss aligns the original image text representations $\mathcal{Z}^I$ and $\mathcal{Z}^T$ by pulling paired representations closer while pushing unpaired ones,

\begin{equation}
\label{equ: INFO_NCE}
L^{I}_{CLIP}(\mathcal{Z^I}, \mathcal{Z^T}) = -\frac{1}{|B|} 
    \sum_{\boldsymbol{z}_i \in \mathcal{Z}^I} \log \frac{\text{exp}(\langle\boldsymbol{z}_i^I, \boldsymbol{z}_i^T\rangle/\tau)}{\sum_{\boldsymbol{z}_j\in \mathcal{Z^T}} \text{exp}(\langle\boldsymbol{z}_i^T, \boldsymbol{z}_i^T\rangle/\tau)}  
 ,
\end{equation}
where $|B|$, $\langle\cdot,\cdot\rangle$, $\tau$ are the batch size, the similarity function, and a learnable temperature to scale the logits, respectively. 
The overall loss $L_{CLIP}$ is the mean of $L_I$ and $L_T$, symmetrical for optimizing the image and text encoders. 
We incorporate the original and augmented representations across modalities in $L_{CLIP}$ to construct the following MVS loss,

\begin{equation}
L_{MVS} = 
    L_{CLIP}(\mathcal{Z}^I, \mathcal{Z}^T)+
    L_{CLIP}(\mathcal{Z}^I, \Tilde{\mathcal{Z}}^T)+
    L_{CLIP}(\Tilde{\mathcal{Z}}^I, \mathcal{Z}^T)+
    L_{CLIP}(\Tilde{\mathcal{Z}}^I, \Tilde{\mathcal{Z}}^T)
,
\end{equation}


\noindent\textbf{SS loss for intra-modal alignment.}
SS loss~\cite{you2023cxr, boecking2022making} aligns representations within modalities. Specifically, we formulate the SS loss as $L_{ISS} = L_{CLIP}(\mathcal{Z}^I, \Tilde{\mathcal{Z}}^I)$ and $L_{TSS} = L_{CLIP}(\mathcal{Z}^T, \Tilde{\mathcal{Z}}^T)$ to align image-image and text-text representations respectively. $L_{ISS}$ pulls the image representations from the same study while pushing the same for different studies. $L_{TSS}$ performs the same for text representations. \textbf{Overall loss.} Thus we optimize the total pre-training objective as: $L = L_{MVS} + \lambda_IL_{ISS} + \lambda_TL_{TSS}$. Here, $\lambda_I$ and $\lambda_T$ are weighting parameters for the image and text SS losses, respectively.


\subsection{CLIP-Factor}
% Grounding, Weak Sup, 
VLM encourages the grounding of the image representations to the textual embeddings. In other words, we deem these textual embeddings as weak labels of the finding attributes, \eg \textit{mass, calcification} \etc~. Thus, we introduce CLIP-Factor, a novel feature attribution method that uses textual descriptions from reports to discover findings-aligned representations. This setup posits a many-to-many mapping between image representations and finding attributes through textual report descriptions. 
Formally, $f^I(\cdot)$ and $f^T(\cdot)$ as the frozen image and text encoders of Mammo-CLIP.
In an image-label dataset, assume $\boldsymbol{x}_i$ and $\boldsymbol{y}_i$ denote the image and $K$-hot vector indicating values of $K$ finding attributes respectively for the $i^{th}$ sample.
We denote image representations as $\boldsymbol{v}_i = \sigma(f^I(\boldsymbol{x}_i))$, where $\sigma: \mathbb{R}^{c \times h \times w} \rightarrow \mathbb{R}^{c \times hw}$ and $c, h$, and $w$ are the channel dimension, height and width of a representation. We denote the mapping function, $\pi^k: \mathbb{R}^{c \times hw} \rightarrow \mathbb{R}^{c \times d}$, signifying the correspondence between a finding attribute $k \in \boldsymbol{y}$ and image representations. Here, $d$ denotes the output representation dimensions. For an arbitrary sample, we use $f^T(\cdot)$ to generate the representations of the textual findings of $k^{th}$ attribute, denoted as $\boldsymbol{t}^k_i \in \mathbb{R}^{d}$, using the positively mentioned prompts, described in Sec. \ref{sec:dataset_aug}. 
\textbf{Training.} Given, $\{\pi^k, \boldsymbol{t}^k\}^K_{k=1}$, we train all the $\pi^k$s using the following contrastive loss,

\begin{equation}
L(\boldsymbol{v}_i, \boldsymbol{y}_i) = -\sum_{k \in \boldsymbol{y_i}}\log
\frac{
    \phi(\pi^k(\boldsymbol{v}_i), \boldsymbol{t}_i^k)
}
{
    \phi(\pi^k(\boldsymbol{v}_i), \boldsymbol{t}_i^k) +
    \sum^{|B|}_{j=1; k\notin \boldsymbol{y_j}}\phi(\pi^k(\boldsymbol{v}_j), \boldsymbol{t}_i^k)
},
\end{equation}

\noindent where $\phi = \exp(\max(\langle a,b \rangle)/\tau)$.
This loss function encourages high similarity between the visual representations $\pi^k(\boldsymbol{v}_i)$ and its corresponding attribute representation $\boldsymbol{t}^k_i$ for images depicting attribute $k$. Conversely, it aims to reduce similarity for images $\boldsymbol{x}_j$ lacking attribute $k$, ensuring that the model accurately discriminates between relevant and non-relevant attributes. After training, we weigh the representations as $\phi(\pi^k(\cdot))f^I(\cdot) \in \mathbb{R}^{h\times w}$ and sum it across the channel dimension to construct the textual aligned heatmap for attribute $k$.

==> sections/method_v4.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{plots/main/Schematic.pdf}
\caption{Schematic view of our method. (a) 
Image-text augmentation for MVS.
% We augment each image-text pair by leveraging different mammogram views and report sections. 
(b) Dataset augmentation by synthesizing reports using image-attribute datasets. (c) Mammo-CLIP pretraining strategy. (d) Feature attribution using Mammo-FACtoR.}
\label{fig:schematic}
\end{center}
\end{figure*}

Our method consists of 3 components: 1) a dual data augmentation strategy augmenting the mammogram-report pairs and integrating mammogram-attribute dataset; 2) an MVS pre-training strategy to align multimodal representations; 3) a novel interpretable feature attribution method to map the textual attributes to the visual features of the image encoder. Assume an image-text dataset $\{(\boldsymbol{x}^I_i, \boldsymbol{x}^T_i)\}_{i=1}^N$, with $N$ is the number of studies in a batch. Also, $f^I(\cdot)$ and $f^T(\cdot)$ is the image and text encoders of Mammo-CLIP.
The schematic of our approach is shown in Fig~\ref{fig:schematic}.

\subsection{Instance and Dataset Augmentation}
\label{sec:dataset_aug}
\noindent\textbf{Image-text augmentation.}
We construct the four pairs using the image-text augmentation strategy: ($\boldsymbol{x}^I, \boldsymbol{x}^T$), ($\boldsymbol{x}^I, A(\boldsymbol{x}^T)$), ($A(\boldsymbol{x}^I), \boldsymbol{x}^T$), and ($A(\boldsymbol{x}^I), A(\boldsymbol{x}^T)$). For brevity, $A$ denotes image and text augmentation. For $i^{th}$ study, $\boldsymbol{x}^I_i$ and $A(\boldsymbol{x}^I_i)$ denote the CC and MLO views respectively.  Likewise, $\boldsymbol{x}^T_i$ and $A(\boldsymbol{x}^T_i)$ denote the impression and findings sections of the report, respectively. We apply similar image and text augmentations for studies without certain views or report sections~\cite{you2023cxr, li2022supervision}.
\noindent\textbf{Dataset augmentation.} To further mitigate the challenge of the limited dataset size, we synthesize reports from the existing mammogram-attribute datasets.
Such datasets consist of a mammogram image paired with a set of attributes \eg \textit{mass, calcification,} \etc~A board-certified radiologist constructs a set of prompts using the values of the attributes (positive, negative \etc). For each sample, we synthesize the report by combining selected prompt sentences, ensuring that the resulting report concatenates text relevant to the attributes identified. We include the prompts in the Appendix.


\subsection{Loss function}

\noindent\textbf{MVS loss for crossmodal alignment.} 
Let $\boldsymbol{Z}^I = \{\boldsymbol{z}^I_i\}_{i=1}^N$ and $\boldsymbol{Z}^T = \{\boldsymbol{z}^T_i\}_{i=1}^N$ be a batch of normalized image and text representations, where $(\boldsymbol{z}^I_i, \boldsymbol{z}^T_i)$ is the representation pair for the original $i^{th}$ study $(\boldsymbol{x^I_i}, \boldsymbol{x^T_i})$. We obtain the normalized representations by projecting the outputs from Mammo-CLIP's image and text encoders, $f^I$ and $f^T$, to the same dimensions, followed by L2 normalization.
Following CLIP~\cite{radford2021learning}, the loss of the image encoder for the $i^{th}$ study is,

%
\begin{equation}
\label{equ: loss_INFO_NCE}
\ell_i^{I}(\boldsymbol{Z}^I, \boldsymbol{Z}^T) =
     \log \frac{\text{exp}(\langle\boldsymbol{z}_i^I, \boldsymbol{z}_i^T \rangle/\tau)}{\sum_{j=1}^N \text{exp}(\langle\boldsymbol{z}_i^I, \boldsymbol{z}_j^T\rangle/\tau)}
 ,
\end{equation}
\noindent where $\langle\cdot,\cdot\rangle$ and $\tau$ are the similarity function and a learnable temperature to scale the logits, respectively. We optimize the text encoder with a symmetrical loss $\ell_i^T$, thus, the total loss $\ell_i$ is the average of $\ell_i^{I}$ and $\ell_i^{T}$. $\ell_i$  aligns $\boldsymbol{Z}^I$ and $\boldsymbol{Z}^T$ by pulling paired representations closer while pushing unpaired ones. 
Assume,
$\Tilde{\boldsymbol{Z}}^I$ and
$\Tilde{\boldsymbol{Z}}^T$ denotes the batch of normalized representations
of the augmented images and text pair, respectively. The MVS~\cite{li2022supervision} strategy leverages cross-modal self-supervision across original and augmented image-text pairs, enhancing generalizability from limited data.
The MVS loss for both the encoders is,

\begin{equation}
\label{equ: loss_MVS}
\ell_i^{MVS} = 
    \ell_i(\boldsymbol{Z}^I, \boldsymbol{Z}^T)+
    \ell_i(\boldsymbol{Z}^I, \Tilde{\boldsymbol{Z}}^T)+
    \ell_i(\Tilde{\boldsymbol{Z}}^I, \boldsymbol{Z}^T)+
    \ell_i(\Tilde{\boldsymbol{Z}}^I, \Tilde{\boldsymbol{Z}}^T)
,
\end{equation}
\noindent\textbf{SS loss for intra-modal alignment.}
We formulate the SS loss~\cite{you2023cxr, boecking2022making} to align the normalized representations within image and text representations as $\ell_i^{ISS} = \ell_i(\boldsymbol{Z}^I, \Tilde{\boldsymbol{Z}}^I)$ and 
$\ell_i^{TSS} = \ell_i(\boldsymbol{Z}^T, \Tilde{\boldsymbol{Z}}^T)$ respectively. $\ell_i^{ISS}$ pulls the image representations from the same study while pushing the same for different studies. $L_{TSS}$ performs the same for text representations. \textbf{Overall loss.} Thus, the final pre-training objective is: $\mathcal{L} = \frac{1}{N}   \sum_{i=1}^N\big(\ell_i^{MVS} + \lambda_I\ell_i^{ISS} + \lambda_T\ell_i^{TSS}\big)$, where, $\lambda_I$ and $\lambda_T$ are the weighting parameters for the image and text SS losses, respectively.


\begin{table*}[t]
\caption{Classification performance on VinDr dataset. 
% We report AUC for calcification, mass, and accuracy for density.
}
\begin{adjustbox}{max width=0.95\textwidth, center}
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{Zero-shot (ZS)}} & 
  \multicolumn{3}{c}{\textbf{Linear Probe (LP)}} &
  \multicolumn{1}{c}{\textbf{Finetune (FT)}} \\ 
\cmidrule(lr){4-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-8}
\multicolumn{1}{l}{\multirow{-2}{*}{\textbf{Label}}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Model}}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Pre-training Data}}} &
  \multicolumn{1}{c}{\scriptsize 100\%} & % Add vertical line after Zero-shot header
  \multicolumn{1}{c}{\scriptsize 10\%} &
  % \multicolumn{1}{c}{\scriptsize 20\%} &
  % \multicolumn{1}{c}{\scriptsize 30\%} &
  \multicolumn{1}{c}{\scriptsize 50\%} &
  \multicolumn{1}{c}{\scriptsize 100\%} &
  \multicolumn{1}{c}{\scriptsize 100\%} \\ 
\midrule
 &
  CLIP w/ RN-50 &
  In-house &
  $0.37$ &
  $0.42$ &
  % $0.43$ &
  % $0.48$ &
  $0.51$ &
  $0.55$ &
  $0.68$ \\
 &
  CLIP w/ EN-B5 &
  In-house &
  $0.53$ &
  $0.53$ &
  % $0.55$ &
  % $0.57$ &
  $0.60$ &
  $0.65$ &
  $0.90$ \\
 % &
 %  Mammo-CLIP w/ RN-101 &
 %  In-house &
 %  $\boldsymbol{0.68}$ &
 %  \underline{$0.91$} &
 %  % $0.91$ &
 %  % $0.92$ &
 %  $0.92$ &
 %  $0.92$ &
 %  $0.96$ \\
 % &
 %  Mammo-CLIP w/ RN-152 &
 %  In-house &
 %  \underline{$0.66$} &
 %  $0.90$ &
 %  % $0.90$ &
 %  % $0.92$ &
 %  $0.92$ &
 %  $0.93$ &
 %  $0.96$ \\
&
  Mammo-CLIP w/ EN-B2  &
  In-house &
  $\boldsymbol{0.68}$ &
  $0.90$ &
  % $0.90$ &
  % $0.91$ &
  $0.92$ &
  $0.92$ &
  $\bm{0.98}$ \\
&
  Mammo-CLIP w/ EN-B5 &
  In-house &
  $0.61$ &
  \underline{$0.91$} &
  % $0.91$ &
  % $0.93$ &
  \underline{$0.93$} &
  \underline{$0.94$} &
  $\bm{0.98}$ \\
\multirow{-5}{*}{Calcification} &
  \cellcolor{lightgray}Mammo-CLIP w/ EN-B5 &
  \cellcolor{lightgray}In-house, VinDr &
  \cellcolor{lightgray}$0.62$ &
  \cellcolor{lightgray}$\bm{0.92}$ &
  % $0.91$ &
  % $0.93$ &
  \cellcolor{lightgray}$\bm{0.94}$ &
  \cellcolor{lightgray}$\bm{0.96}$ &
  \cellcolor{lightgray}$\bm{0.98}$ \\
\midrule
&
  CLIP w/ RN-50 &
  In-house &
  $0.20$ &
  $0.34$ &
  % $0.43$ &
  % $0.48$ &
  $0.42$ &
  $0.49$ &
  $0.57$ \\
 &
  CLIP w/ EN-B5 &
  In-house &
  $0.32$ &
  $0.52$ &
  % $0.55$ &
  % $0.57$ &
  $0.57$ &
  $0.59$ &
  $0.78$ \\
 % &
 %  Mammo-CLIP w/ RN-101 &
 %  In-house &
 %  $0.40$ &
 %  $0.62$ &
 %  % $0.91$ &
 %  % $0.92$ &
 %  $0.69$ &
 %  $0.71$ &
 %  $0.78$ \\
 % &
 %  Mammo-CLIP w/ RN-152 &
 %  In-house &
 %  $0.48$ &
 %  $0.68$ &
 %  % $0.90$ &
 %  % $0.91$ &
 %  $0.73$ &
 %  $0.74$ &
 %  $0.80$ \\
&
  Mammo-CLIP w/ EN-B2 &
  In-house &
  \underline{$0.58$} &
  $0.69$ &
  % $0.90$ &
  % $0.91$ &
  $0.72$ &
  $0.73$ &
  \underline{$0.85$} \\
&
  Mammo-CLIP w/ EN-B5 &
  In-house &
  $0.48$ &
  \underline{$0.73$} &
  % $0.91$ &
  % $0.93$ &
  \underline{$0.78$} &
  \underline{$0.79$} &
  \underline{$0.85$} \\
\multirow{-6}{*}{Mass} &
  \cellcolor{lightgray}Mammo-CLIP w/ EN-B5 &
  \cellcolor{lightgray}In-house, VinDr &
  \cellcolor{lightgray}$\bm{0.76}$ &
  \cellcolor{lightgray}$\bm{0.80}$ &
  % $0.91$ &
  % $0.93$ &
  \cellcolor{lightgray}$\bm{0.84}$ &
  \cellcolor{lightgray}$\bm{0.86}$ &
  \cellcolor{lightgray}$\bm{0.88}$ \\
\midrule
&
  CLIP w/ RN-50 &
  In-house &
  $0.04$ &
  $0.55$ &
  % $0.43$ &
  % $0.48$ &
  $0.61$ &
  $0.69$ &
  $0.72$ \\
 &
  CLIP w/ EN-B5 &
  In-house &
  $0.10$ &
  $0.76$ &
  % $0.55$ &
  % $0.57$ &
  $0.76$ &
  $0.78$ &
  $0.83$ \\
 % &
 %  Mammo-CLIP w/ RN-101 &
 %  In-house &
 %  \underline{$0.16$} &
 %  $0.77$ &
 %  % $0.91$ &
 %  % $0.92$ &
 %  $0.79$ &
 %  $0.82$ &
 %  $0.84$ \\
 % &
 %  Mammo-CLIP w/ RN-152 &
 %  In-house &
 %  \bm{$0.17$} &
 %  $0.77$ &
 %  % $0.90$ &
 %  % $0.92$ &
 %  $0.79$ &
 %  $0.84$ &
 %  $0.85$ \\
&
  Mammo-CLIP w/ EN-B2 &
  In-house &
  $0.13$ &
  \underline{$0.80$} &
  % $0.91$ &
  % $0.93$ &
  $0.82$ &
  $0.84$ &
  \underline{$0.85$} \\
&
  Mammo-CLIP w/ EN-B5 &
  In-house &
  $0.15$ &
  $\bm{0.83}$ &
  % $0.91$ &
  % $0.93$ &
  \underline{$0.84$} &
  \underline{$0.85$} &
  $\bm{0.88}$ \\
\multirow{-6}{*}{Density} &
  \cellcolor{lightgray}Mammo-CLIP w/ EN-B5 &
  \cellcolor{lightgray}In-house, VinDr &
  \cellcolor{lightgray}$0.15$ &
  \cellcolor{lightgray}$\bm{0.83}$ &
  % $0.91$ &
  % $0.93$ &
  \cellcolor{lightgray}$\bm{0.86}$ &
  \cellcolor{lightgray}$\bm{0.86}$ &
  \cellcolor{lightgray}$\bm{0.88}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{table:classification_vindr_cls}
\end{table*}

\subsection{Mammo-FActOR}
% Grounding, Weak Sup, 
Mammo-CLIP aligns the image and text representations. In other words, we deem the text representations as weak labels of the attributes, \eg \textit{mass, calcification} \etc~Thus, we introduce Mammo-FActOR, a novel feature attribution method that uses textual descriptions from reports to discover attributes-aligned representations. We leverage many-to-many mapping between image representations and attributes through the report. 
% We freeze the encoders $f^I(\cdot)$ and $f^T(\cdot)$ throughout this method.
Assume $\boldsymbol{x}_i$ and $\boldsymbol{y}_i$ denote the image and $K$-hot vector indicating values of $K$ attributes respectively for the $i^{th}$ sample in a dataset.
We obtain image representation from the frozen image encoder as $\boldsymbol{v}_i = \sigma(f^I(\boldsymbol{x}_i))$, where $\sigma: \mathbb{R}^{c \times h \times w} \rightarrow \mathbb{R}^{c \times hw}$ and $c, h$, and $w$ are the channel dimension, height and width of a representation. We denote the mapping function, $\pi^k: \mathbb{R}^{c \times hw} \rightarrow \mathbb{R}^{c \times d}$, signifying the correspondence between an attribute $k \in \boldsymbol{y}$ and image representations. Here, $d$ denotes the output representation dimensions. Also for the $i^{th}$ sample, we use the frozen $f^T(\cdot)$ to generate the representations of the textual attributes of $k^{th}$ attribute, denoted as $\boldsymbol{t}^k_i \in \mathbb{R}^{d}$, using the positively mentioned prompts, described in Sec. \ref{sec:dataset_aug}. 
\textbf{Training.} Given, $\{\pi^k, \boldsymbol{t}^k\}^K_{k=1}$, we train all the $\pi^k$s using the following loss,

\begin{equation}
L(\boldsymbol{v}_i, \boldsymbol{y}_i) = -\sum_{k \in \boldsymbol{y_i}}\log
\frac{
    \phi(\pi^k(\boldsymbol{v}_i), \boldsymbol{t}_i^k)
}
{
    \phi(\pi^k(\boldsymbol{v}_i), \boldsymbol{t}_i^k) +
    \sum^{|B|}_{j=1; k\notin \boldsymbol{y_j}}\phi(\pi^k(\boldsymbol{v}_j), \boldsymbol{t}_i^k)
},
\end{equation}

\noindent where $\phi = \exp(\max(\langle a,b \rangle)/\tau)$.
This contrastive loss encourages high similarity between embedding of the visual representations $\pi^k(\boldsymbol{v}_i)$ and its corresponding attribute representation $\boldsymbol{t}^k_i$ for attribute $k$. Conversely, it aims to reduce similarity for images $\boldsymbol{x}_j$ lacking attribute $k$, ensuring that the model accurately discriminates between relevant and non-relevant attributes. 
\textbf{Feature attribution.} After training, we weigh the representations as, $\phi(\pi^k(\cdot))f^I(\cdot) \in \mathbb{R}^{h\times w}$ and sum it across the channel dimension to construct the textual aligned heatmap for attribute $k$.

==> sections/results_v0.tex <==
\begin{table*}[h]
% \caption{AUCROC}
% \begin{adjustbox}{max width=0.95\textwidth, center}
% \begin{tabular}{lccc|ccccc|c}
% \toprule
% \multicolumn{1}{c}{} &
%   \multicolumn{1}{c}{} &
%   \multicolumn{1}{c}{} &
%   \multicolumn{1}{c|}{\textbf{Zero-shot}} & 
%   \multicolumn{5}{c|}{\textbf{Linear Probe}} &
%   \multicolumn{1}{c}{\textbf{Finetune}} \\ 
% \cmidrule(lr){4-4}
% \cmidrule(lr){5-9}
% \cmidrule(lr){10-10}
% \multicolumn{1}{l}{\multirow{-2}{*}{\textbf{Label}}} &
%   \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Model}}} &
%   \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Pre-training Data}}} &
%   \multicolumn{1}{c|}{\scriptsize 100\%} & % Add vertical line after Zero-shot header
%   \multicolumn{1}{c}{\scriptsize 10\%} &
%   \multicolumn{1}{c}{\scriptsize 20\%} &
%   \multicolumn{1}{c}{\scriptsize 30\%} &
%   \multicolumn{1}{c}{\scriptsize 50\%} &
%   \multicolumn{1}{c|}{\scriptsize 100\%} &
%   \multicolumn{1}{c}{\scriptsize 100\%} \\ 
% \midrule
%  &
%   CLIP w/ ResNet-50 &
%   In-house &
%   $0.37$ &
%   $0.42$ &
%   $0.43$ &
%   $0.48$ &
%   $0.51$ &
%   $0.55$ &
%   $0.68$ \\
%  &
%   CLIP w/ EfficientNet-B5 &
%   In-house &
%   $0.53$ &
%   $0.53$ &
%   $0.55$ &
%   $0.57$ &
%   $0.60$ &
%   $0.65$ &
%   $0.90$ \\
%  &
%   Mammo-CLIP w/ ResNet-101 &
%   In-house &
%   $0.68$ &
%   $0.91$ &
%   $0.91$ &
%   $0.92$ &
%   $0.92$ &
%   $0.92$ &
%   $0.96$ \\
%  &
%   Mammo-CLIP w/ ResNet-152 &
%   In-house &
%   $0.66$ &
%   $0.90$ &
%   $0.90$ &
%   $0.92$ &
%   $0.92$ &
%   $0.93$ &
%   $0.96$ \\
% &
%   Mammo-CLIP w/ EfficientNet-B2 &
%   In-house &
%   $0.68$ &
%   $0.90$ &
%   $0.90$ &
%   $0.91$ &
%   $0.92$ &
%   $0.92$ &
%   $0.98$ \\
% \multirow{-5}{*}{Suspicious  Calcification} &
%   Mammo-CLIP w/ EfficientNet-B5 &
%   In-house &
%   $0.61$ &
%   $0.91$ &
%   $0.91$ &
%   $0.93$ &
%   $0.93$ &
%   $0.94$ &
%   $0.98$ \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{table:classification_vindr}
% \end{table*}
